CONFIGEN: A tool for managing configuration options

This paper introduces CONFIGEN, a tool that helps modularizing software. CONFIGEN allows the developer to select a set of elementary components for his software through an interactive interface. Configuration files for use by C/assembly code and Makefiles are then automatically generated, and we successfully used it as a helper tool for complex system software refactoring. CONFIGEN is based on propositional logic, and its implementation faces hard theoretical problems.

==> eptcsdata.tex <==
\providecommand{\event}{I. Lynce and R. Treinen (eds.): Workshop on\\
Logics for Component Configuration (LoCoCo 2010)}
\providecommand{\volume}{29}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{32}
\providecommand{\eid}{4}
\providecommand{\publicationstatus}{I. Lynce and R. Treinen (eds.): Workshop on\\
Logics for Component Configuration (LoCoCo 2010)\\
EPTCS 29, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.29.4}{10.4204/EPTCS.29.4}}
\pdfoutput=1

